NCRF: Neural Contact Radiance Fields for Free-Viewpoint Rendering of Hand-Object Interaction

Modeling hand-object interactions is a fundamentally challenging task in 3D computer vision. Despite remarkable progress that has been achieved in this field, existing methods still fail to synthesize the hand-object interaction photo-realistically, suffering from degraded rendering quality caused by the heavy mutual occlusions between the hand and the object, and inaccurate hand-object pose estimation. To tackle these challenges, we present a novel free-viewpoint rendering framework, Neural Contact Radiance Field (NCRF), to reconstruct hand-object interactions from a sparse set of videos. In particular, the proposed NCRF framework consists of two key components: (a) A contact optimization field that predicts an accurate contact field from 3D query points for achieving desirable contact between the hand and the object. (b) A hand-object neural radiance field to learn an implicit hand-object representation in a static canonical space, in concert with the specifically designed hand-object motion field to produce observation-to-canonical correspondences. We jointly learn these key components where they mutually help and regularize each other with visual and geometric constraints, producing a high-quality hand-object reconstruction that achieves photo-realistic novel view synthesis. Extensive experiments on HO3D and DexYCB datasets show that our approach outperforms the current state-of-the-art in terms of both rendering quality and pose estimation accuracy.

==> Figure/supply_conanical_mlp/item.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{Figure/supply_conanical_mlp/Canonical_MLP.pdf}
\caption{
The network architecture of canonical neural radiance field. }
\label{fig:canonical_mlp}
\end{figure}

==> Figure/supply_more_results_multi_view/item.tex <==
\begin{figure*}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{Figure/supply_more_results_multi_view/More_Results_Multi.pdf}
\caption{
Qualitative comparison with HumanNeRF~\cite{weng2022humannerf} on the HO3D dataset.
}
\label{fig:supply_more_result_multi_view}
\end{figure*}

==> Figure/supply_more_results_single_view/item.tex <==
\begin{figure*}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{Figure/supply_more_results_single_view/More_Results_Single.pdf}
\caption{
Qualitative comparison with HumanNeRF~\cite{weng2022humannerf} on monocular video.
}
\label{fig:supply_more_result_single_view}
\end{figure*}

==> Figure/supply_motion_mlp/item.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{Figure/supply_motion_mlp/Motion_MLP.pdf}
\caption{
The schematic diagram of the modules in the NCRF pipeline: 
(a) Rigid object Pose correction module. 
(b) Hand joint rotation correction module. 
(c) Non-rigid motion module.}
\label{fig:motion_mlp}
\end{figure}

==> Table/ablation_num_view/item.tex <==
\begin{table}[t]
  \caption{Comparison of models trained with different numbers
of camera views on HO3D~\cite{hampali2020honnotate} datasets.} %LPIPS* = LPIPS $\times 10^3$}
  \label{table:ab_num_view}
  % \scriptsize
  \small
  % \footnotesize
  % \normalsize
  \centering
  \setlength\tabcolsep{3pt}
  \begin{tabular}{ l |c| c| c}
    \toprule
     &\textbf{PSNR}$\uparrow$  &\textbf{SSIM}$\uparrow$ &\textbf{LPIPS*}$\downarrow$\\
    \midrule
    3 views & \textbf{29.74} & \textbf{0.9758}    & \textbf{32.47}\\
    2 views & 29.57 & 0.9732    & 33.01 \\
    1 view & 27.93 &0.9704    & 35.85 \\
    \bottomrule
  \end{tabular}
\end{table}

==> Table/comparison/item.tex <==
% \begin{table*}
%   \caption{Detailed quantitative results of free-viewpoint rendering and hand-object pose optimization on HO3Dv3~\cite{hampali2020honnotate} and DexYCB~\cite{chao2021dexycb} datasets in PSNR $\uparrow$,
% SSIM $\uparrow$, ADD-0.1D $\uparrow$ (higher is better), and LPIPS $\downarrow$, MPJPE $\downarrow$, IV $\downarrow$ (lower is better). Our method outperforms in both datasets, compared to the baseline HOGAN~\cite{hu2022hand} (GAN) and HumanNeRF~\cite{weng2022humannerf} (HN) in terms of rendering quality, and ContactOpt~\cite{grady2021contactopt} (CO) in terms of pose accuracy. Hasson~\etal~\cite{hasson2020leveraging} (IN) is the initial pose estimator. }
%   \label{table:corruption_type}
%   \scriptsize
%   % \small
%   % \footnotesize
%   % \normalsize
%   \centering
%   \setlength\tabcolsep{3pt}
%   \begin{tabular}{c | c |ccc | ccc | ccc | ccc | ccc | ccc}
%     \toprule
%     \multirow{3}{*}{Datasets} & \multirow{3}{*}{Objects}
%      & \multicolumn{9}{c|}{Free-viewpoint Rendering} & \multicolumn{9}{c}{Pose Optimization}\\
%      & & \multicolumn{3}{c}{PSNR$\uparrow$}  & \multicolumn{3}{c}{SSIM$\uparrow$}  & \multicolumn{3}{c|}{LPIPS$\downarrow$} & \multicolumn{3}{c}{MPJPE$\downarrow$}  & \multicolumn{3}{c}{ADD-0.1D$\uparrow$}  & \multicolumn{3}{c}{IV$\downarrow$}   \\
%        & & GAN & HN & Ours & GAN & HN & Ours &GAN &HN & Ours &IN & CO & Ours &IN & CO & Ours &IN & CO & Ours  \\
%     \midrule
%     \multirow{6}{*}{HO3Dv3}
%     &\emph{power\_drill}& 29.1 & 0.967 &40.9   & 29.1 & 0.967 &40.9  & 29.1 & 0.967 &40.9 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2  \\
%     &\emph{bleach\_cleanser}& 29.1 & 0.967 &40.9   & 29.1 & 0.967 &40.9  & 29.1 & 0.967 &40.9 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2  \\
%     &\emph{scissors}& 29.1 & 0.967 &40.9   & 29.1 & 0.967 &40.9  & 29.1 & 0.967 &40.9 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2  \\
%     &\emph{potted\_meat\_can}& 29.1 & 0.967 &40.9   & 29.1 & 0.967 &40.9  & 29.1 & 0.967 &40.9 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2  \\
%     &\emph{banana}& 30.57 & 30.57 &30.57   & 0.9795 & 0.9795 &0.9795  & 31.60 & 31.60 &31.60  &10.51 &10.51 & 10.51 &90.71 &90.71 & 90.71 &9.21 &9.21 & 9.21  \\
%     \cmidrule{2-20}
%      &\emph{average} & 29.1 & 0.967 &40.9   & 29.1 & 0.967 &40.9  & 29.1 & 0.967 &40.9 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2  \\
%      \midrule
%      \multirow{6}{*}{DexYCB}
%      &\emph{tuna\_fish\_can}& 29.1 & 0.967 &40.9   & 29.1 & 0.967 &40.9  & 29.1 & 0.967 &40.9 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2  \\
%      &\emph{pitcher\_base}& 29.1 & 0.967 &40.9   & 29.1 & 0.967 &40.9  & 29.1 & 0.967 &40.9 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2  \\
%      &\emph{mustard\_bottle}& 29.1 & 0.967 &40.9   & 29.1 & 0.967 &40.9  & 29.1 & 0.967 &40.9 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2  \\
%     &\emph{mug}& 29.1 & 0.967 &40.9   & 29.1 & 0.967 &40.9  & 29.1 & 0.967 &40.9 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2  \\
%     &\emph{sugar\_box}& 29.1 & 0.967 &40.9   & 29.1 & 0.967 &40.9  & 29.1 & 0.967 &40.9 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2  \\
%     \cmidrule{2-20}
%      &average & 29.1 & 0.967 &40.9   & 29.1 & 0.967 &40.9  & 29.1 & 0.967 &40.9 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2 &10.5 &90.7 & 9.2  \\
     
%     \bottomrule
%   \end{tabular}
% \end{table*}

\begin{table*}
  \caption{Detailed quantitative results of free-viewpoint rendering and hand-object pose optimization on HO3Dv3~\cite{hampali2020honnotate} and DexYCB~\cite{chao2021dexycb} datasets in PSNR $\uparrow$,
SSIM $\uparrow$, ADD-0.1D $\uparrow$ (higher is better), and LPIPS $\downarrow$, MPJPE $\downarrow$, IV $\downarrow$ (lower is better). Our method outperforms in both datasets, compared to the baseline HumanNeRF~\cite{weng2022humannerf} in terms of rendering quality, and ContactOpt~\cite{grady2021contactopt} (ContOpt) in terms of pose accuracy. Hasson~\etal~\cite{hasson2020leveraging} is the initial pose estimator. }
  \label{table:corruption_type}
  \scriptsize
  % \small
  % \footnotesize
  % \normalsize
  \centering
  \setlength\tabcolsep{3pt}
  \begin{tabular}{c | c |cc | cc | cc | ccc | ccc | ccc}
    \toprule
    \multirow{3}{*}{\textbf{Datasets}} & \multirow{3}{*}{\textbf{Objects}}
     & \multicolumn{6}{c|}{\textbf{Free-viewpoint Rendering}} & \multicolumn{9}{c}{\textbf{Pose Optimization}}\\
     & & \multicolumn{2}{c}{PSNR$\uparrow$}  & \multicolumn{2}{c}{SSIM$\uparrow$}  & \multicolumn{2}{c|}{LPIPS$\downarrow$} & \multicolumn{3}{c}{MPJPE$\downarrow$}  & \multicolumn{3}{c}{ADD-0.1D$\uparrow$}  & \multicolumn{3}{c}{IV$\downarrow$}   \\
       & & HumanNeRF & Ours & HumanNeRF & Ours &HumanNeRF & Ours &\cite{hasson2020leveraging} & ContOpt & Ours &\cite{hasson2020leveraging} & ContOpt & Ours &\cite{hasson2020leveraging} & ContOpt & Ours  \\
    \midrule
    \multirow{6}{*}{HO3Dv3}
    &\emph{power\_drill} & 30.57 &29.25    & 0.9795 &0.9717   & 31.60 &37.19  &10.51 &10.51 & 10.51 &90.71 &90.71 & 90.71 &9.21 &9.21 & 9.21  \\
    &\emph{bleach\_cleanser}& 30.57 &30.57    & 0.9795 &0.9795   & 31.60 &31.60  &10.51 &10.51 & 10.51 &90.71 &90.71 & 90.71 &9.21 &9.21 & 9.21  \\
    &\emph{scissors}& 30.57 &29.48    & 0.9795 &0.9767   & 31.60 &30.72  &10.51 &10.51 & 10.51 &90.71 &90.71 & 90.71 &9.21 &9.21 & 9.21  \\
    &\emph{potted\_meat\_can}& 30.57 &30.57    & 0.9795 &0.9795   & 31.60 &31.60  &10.51 &10.51 & 10.51 &90.71 &90.71 & 90.71 &9.21 &9.21 & 9.21  \\
    &\emph{banana} & 30.57 &30.58    & 0.9795 &0.9795   & 31.60 &31.60  &10.51 &10.51 & 10.51 &90.71 &90.71 & 90.71 &9.21 &9.21 & 9.21  \\
    \cmidrule{2-17}
     &\emph{average} & 30.57 &30.57    & 0.9795 &0.9795   & 31.60 &31.60  &10.51 &10.51 & 10.51 &90.71 &90.71 & 90.71 &9.21 &9.21 & 9.21  \\
     \midrule
     \multirow{6}{*}{DexYCB}
     &\emph{tuna\_fish\_can}& 30.57 &30.57    & 0.9795 &0.9795   & 31.60 &31.60  &10.51 &10.51 & 10.51 &90.71 &90.71 & 90.71 &9.21 &9.21 & 9.21  \\
     &\emph{pitcher\_base}& 30.57 &30.57    & 0.9795 &0.9795   & 31.60 &31.60  &10.51 &10.51 & 10.51 &90.71 &90.71 & 90.71 &9.21 &9.21 & 9.21  \\
     &\emph{mustard\_bottle}& 30.57 &30.57    & 0.9795 &0.9795   & 31.60 &31.60  &10.51 &10.51 & 10.51 &90.71 &90.71 & 90.71 &9.21 &9.21 & 9.21  \\
    &\emph{mug}& 30.57 &30.57    & 0.9795 &0.9795   & 31.60 &31.60  &10.51 &10.51 & 10.51 &90.71 &90.71 & 90.71 &9.21 &9.21 & 9.21  \\
    &\emph{sugar\_box}& 30.57 &30.57    & 0.9795 &0.9795   & 31.60 &31.60  &10.51 &10.51 & 10.51 &90.71 &90.71 & 90.71 &9.21 &9.21 & 9.21  \\
    \cmidrule{2-17}
     &average & 30.57 &30.57    & 0.9795 &0.9795   & 31.60 &31.60  &10.51 &10.51 & 10.51 &90.71 &90.71 & 90.71 &9.21 &9.21 & 9.21  \\
     
    \bottomrule
  \end{tabular}
\end{table*}

==> Table/supply_dataset/item.tex <==
\begin{table}[t]
  \caption{Training and test split of each
objects of the HO3D~\cite{qian2022arnnotate} dataset for free-viewpoint rendering. }
  \label{table:supply_dataset}
  \scriptsize
  % \small
  % \footnotesize
  % \normalsize
  \centering
  \setlength\tabcolsep{3pt}
  \begin{tabular}{c | c |c| c}
    \toprule
    \textbf{Datasets} &\textbf{Objects}
    &\textbf{Train}  &\textbf{Test} \\
    \midrule
    \multirow{5}{*}{HO3D}
    &\emph{power\_drill} & MDF10, MDF11, MDF13 & MDF12, MDF14  \\
    &\emph{bleach\_cleanser} & ABF11, ABF12, GSF13 & ABF10, ABF14  \\
    &\emph{scissors} & GSF12, GSF13, GSF14 & GSF10, GSF11 \\
    &\emph{potted\_meat\_can} & GPMF12, GPMF13, GPMF14 & GPMF10, GPMF11  \\
    &\emph{banana} & SiBF10, SiBF12, SiBF14 & SiBF11, SiBF13  \\
    \midrule
    \multirow{2}{*}{DexYCB}
    &\multirow{2}{*}{all} 
    & 841412060263, 932122060861 &\multirow{2}{*}{all other views}\\
    &&932122062010   \\
    \bottomrule
  \end{tabular}
\end{table}

==> Table/supply_more_results/item.tex <==
\begin{table}[t]
  \caption{Detailed quantitative results of free-viewpoint rendering on HO3D~\cite{hampali2020honnotate} and DexYCB~\cite{chao2021dexycb} datasets in PSNR $\uparrow$,
SSIM $\uparrow$ (higher is better), and LPIPS $\downarrow$ (lower is better). HumanNeRF~\cite{weng2022humannerf} is used as the baseline method in comparison. }
  \label{table:supply_more_results}
  \scriptsize
  \centering
  \setlength\tabcolsep{3pt}
  \begin{tabular}{c | c |cc | cc | cc }
    \toprule
    \multirow{2}{*}{\textbf{Datasets}} & \multirow{2}{*}{\textbf{Object}}
     & \multicolumn{2}{c|}{\textbf{PSNR}$\uparrow$}  & \multicolumn{2}{c|}{\textbf{SSIM}$\uparrow$}  & \multicolumn{2}{c}{\textbf{LPIPS*}$\downarrow$} \\
       & & \cite{weng2022humannerf} & Ours & \cite{weng2022humannerf} & Ours &\cite{weng2022humannerf} & Ours\\
    \midrule
    \multirow{6}{*}{HO3D}
    &\emph{035-power-drill} &25.95  &\textbf{29.25}    &0.9703  &\textbf{0.9717}  &40.16  &\textbf{33.19}\\
    &\emph{021-bleach-cleanser}&25.01  &\textbf{30.11}   &0.9632  &\textbf{0.9786 }  & 41.07 &\textbf{32.71}\\
    &\emph{037-scissors}&27.77  &\textbf{29.48}   &0.9675  &\textbf{0.9767} &35.96  &\textbf{30.72}\\
    &\emph{010-potted-meat-can}&25.63  &\textbf{29.30}    &0.9614  &\textbf{0.9724 }  &43.80  &\textbf{34.15} \\
    &\emph{011-banana} &25.95  &\textbf{30.58}    &0.9703  &\textbf{0.9795}  &40.16  &\textbf{31.60}\\
    \cmidrule{2-8}
     &\emph{average} &26.06  &\textbf{29.74}    &0.9665  &\textbf{0.9758}   & 40.23 &\textbf{32.47} \\
     \midrule
     \multirow{6}{*}{DexYCB}
     &\emph{007-tuna-fish can}&25.32  &\textbf{32.42}    &0.9631  &\textbf{0.9786 }  &26.10  &\textbf{22.50} \\
     &\emph{019-pitcher-base}&26.96  &\textbf{33.21}    &0.9725  &\textbf{0.9849}   &25.03  &\textbf{19.72} \\
     &\emph{006-mustard-bottle}&29.95  &\textbf{32.95}    &0.9766  &\textbf{0.9837}   &26.48  &\textbf{20.45} \\
    &\emph{025-mug}&30.04  &\textbf{33.75 }   &0.9715  &\textbf{0.9853}   &29.31  &\textbf{17.64} \\
    &\emph{004-sugar-box}&24.31  &\textbf{28.50}    &0.9628  &\textbf{0.9741 }  &30.23  &\textbf{21.54} \\
    \cmidrule{2-8}
     &average &27.32  &\textbf{32.16}    &0.9719  &\textbf{0.9813 }  &27.43 &\textbf{20.37} \\
     
    \bottomrule
  \end{tabular}
\end{table}
